Variational Quantum Algorithms in the era of Early Fault Tolerance

Quantum computing roadmaps predict the availability of 10,000 qubit devices within the next 3-5 years. With projected two-qubit error rates of 0.1%, these systems will enable certain operations under quantum error correction (QEC) using lightweight codes, offering significantly improved fidelities compared to the NISQ era. However, the high qubit cost of QEC codes like the surface code (especially at near-threshold physical error rates) limits the error correction capabilities of these devices. In this emerging era of Early Fault Tolerance (EFT), it will be essential to use QEC resources efficiently and focus on applications that derive the greatest benefit. In this work, we investigate the implementation of Variational Quantum Algorithms in the EFT regime (EFT-VQA). We introduce partial error correction (pQEC), a strategy that error-corrects Clifford operations while performing Rz rotations via magic state injection instead of the more expensive T-state distillation. Our results show that pQEC can improve VQA fidelities by 9.27x over standard approaches. Furthermore, we propose architectural optimizations that reduce circuit latency by ~2x, and achieve qubit packing efficiency of 66% in the EFT regime.

==> ISCA2025ACMtemplate/sections/Clarifications.tex <==
\section*{\revision{Revision Cover Letter}}\label{sec:rev_cover}

\revision{
The authors would like to thank the reviewers for their insightful feedback. Before addressing specific questions, we would like to emphasize the timeliness and potential impact of this work.  
Coinciding with our submission, John Preskill introduced his vision for the post-NISQ era with Megaquop quantum systems, aiming to execute a million quantum operations with error rates of $10^{-6}$ per logical gate. As Preskill outlined, these systems should integrate quantum error correction (QEC) with NISQ-inspired techniques, targeting approximately 100 logical qubits (supported by thousands of physical qubits) and circuit depths of $\sim10,000$, thereby surpassing the limitations of both classical and NISQ approaches. Our vision for the emerging EFT era, as discussed in this paper, aligns closely with this perspective. Identifying meaningful quantum applications for this era is crucial, and our work makes a compelling case for the utility of Variational Quantum Algorithms (VQAs).  
To quantitatively assess our proposal, we primarily focus on quantum systems with around 10,000 physical qubits and a physical error rate of $10^{-3}$. We clearly demonstrate the advantages of a partial QEC approach over conventional QEC on a Clifford+T gate-set. This revision further expands on the superior benefits of our approach compared to alternative methods. However, we stress that the advantages of our work are not confined to 10k-qubit EFT systems alone. Our methodology remains beneficial for quantum systems of any size, particularly when executing a broad range of applications—such as VQAs—that exhibit some level of algorithmic error tolerance and push the limits of device capabilities.  
For instance, on a 10,000-qubit device, our method could perhaps enable running a 50-logical-qubit problem with the same fidelity that a conventional fault-tolerant quantum computing (FTQC) approach would achieve on a 25-logical-qubit problem. Similarly, on a 100,000-qubit device, our method could perhaps support a 200-logical-qubit problem with the same fidelity as conventional FTQC on a 100-logical-qubit problem. This capability is crucial, as it allows us to push applications further along the frontier of practical quantum utility.  
This efficiency is especially significant given the substantial costs associated with large-scale quantum systems. A 10k–100k-qubit machine would require investments in the range of multiple billions of dollars, considering expenses related to electronics, power, and infrastructure. From a practical standpoint, maximizing the computational utility of such an expensive system is essential to achieving a favorable return on investment. Our methodology directly supports this goal by enabling the execution of larger, more impactful use cases on these eventual state-of-the-art quantum platforms.} 

\subsection{\revision{Common}}
\begin{enumerate}
    \item \question{Scalability beyond 10k qubits: }\revision{Refer to section \ref{subsec:scalability}}
    \item \question{Justification of layout and suitability for VQAs} \revision{Refer to section \ref{subsec:good_layout}}
    \item \revision{We would like to point out a change in Figure \ref{fig:blocked_all_to_all_vs_hardware_efficient} and the corresponding data. This experiment was rerun using better simulation methodology - more shots and a more aggressive optimization technique, which gave us improved results. Note that the qualitative takeaway from the plot remains unchanged, only the numbers have slightly changed. We also did general rewriting of the paper (keeping the technical content unchanged) to keep things within the acceptable page limit. We are not highlighting these changes.}
\end{enumerate}


\subsection{\textcolor{blue}{Rev A}}
\begin{enumerate}
    \item \question{Accounting for variable angle rotations: }\revision{Refer to section \ref{subsec:good_layout} and figure \ref{fig:tile_layout}.} 
    \item \question{Suitability of layout for VQAs: }\revision{Common 2}
    \item \question{Impact of proposed techniques on execution time.} \revision{Refer to Sections \ref{subsec:good_layout}, \ref{subsec:patch_shuffling}, \ref{subsec:layout_aware_ansatz}. In \ref{subsec:layout_aware_ansatz}, we show an explicit reduction in execution time in Table \ref{tab:time}. For \ref{subsec:patch_shuffling}, and \ref{subsec:good_layout}, we show a space-time volume comparison since there exists a space and time trade-off for these parameters. By overprovisioning the space, we can reduce time further, however that affects other important parameters (like packing efficiency) which is not desirable.}
    \item \question{Does the post-processing phase of magic-state injection introduce additional complexity? } \revision{If the magic state consumption fails, we have to inject a new state and repeat the process till consumption succeeds. This is the additional post-processing complexity introduced by magic state injection. However, all data presented in the paper accounts for this post-processing complexity. We account for this while mathematically proving the correctness of Patch shuffling as well (see section \ref{sec:appendix})}
    \item \question{Effectiveness of techniques for more than 10k qubits: }\revision{Common 1}
\end{enumerate}

\subsection{\textcolor{blue}{Rev B}}
\begin{enumerate}
    \item \question{Baseline and comparison with SOTA error mitigation techniques: }\revision{The current baseline is a VQA implementation assuming fully-connected hardware. We assume no additional swaps or connectivity constraints which eliminates all routing error in the NISQ case}
    \item \question{Comparison with SOTA NISQ error mitigation techniques: }\revision{Refer to section \ref{sec:related_work}}
    \item \question{Justification of layout: }\revision{Common 2}
    \item \question{Feasibility of Rz hardware implementation: }\revision{Common 1}
\end{enumerate}

\subsection{\textcolor{blue}{Rev C}}
\begin{enumerate}
    \item \question{Using Geometric Mean Instead of Arithmetic Mean: }\revision{All numbers have been re-evaluated using Geo-mean. Highlighted in blue throughout the text}
    \item \question{Proof of Patch Shuffling }\revision{Refer to section \ref{sec:appendix}}
\end{enumerate}


% \ms{Since we are gonna be cutting/rewriting content, make sure that we mention somewhere that we did ``general rewriting''}
